Optimal strategies in concurrent reachability games

We study two-player reachability games on finite graphs. At each state the interaction between the players is concurrent and there is a stochastic Nature. Players also play stochastically. The literature tells us that 1) Player B, who wants to avoid the target state, has a positional strategy that maximizes the probability to win (uniformly from every state) and 2) from every state, for every {\epsilon} > 0, Player A has a strategy that maximizes up to {\epsilon} the probability to win. Our work is two-fold. First, we present a double-fixed-point procedure that says from which state Player A has a strategy that maximizes (exactly) the probability to win. This is computable if Nature's probability distributions are rational. We call these states maximizable. Moreover, we show that for every {\epsilon} > 0, Player A has a positional strategy that maximizes the probability to win, exactly from maximizable states and up to {\epsilon} from sub-maximizable states. Second, we consider three-state games with one main state, one target, and one bin. We characterize the local interactions at the main state that guarantee the existence of an optimal Player A strategy. In this case there is a positional one. It turns out that in many-state games, these local interactions also guarantee the existence of a uniform optimal Player A strategy. In a way, these games are well-behaved by design of their elementary bricks, the local interactions. It is decidable whether a local interaction has this desirable property.

==> Tex/CorrectGameForms.tex <==
%!TEX root = ../lipics-v2021-sample-article

\smallskip \noindent \textbf{Correct Game Forms.}
%We have %defined the correct game forms and 
%proved that correct game forms exactly correspond to the game forms that, used in any concurrent reachability, ensure that all states are optimal. %In this section, we study such game forms: first, we some properties on game forms that are sufficient for them to be correct, second we look at the problem if a game form is correct and show that this can be done by using the existential theory of the reals.
%Let us now 
%\subsection{Sufficient conditions for correctness}
%However, 
The definition of correct game forms involves a universal quantification over partial valuations and a least fixed point operator. Thus, it is not straightforward to visualize what this notion %of correct game forms 
encompasses. Here, we give a sufficient condition for game forms to be correct and deduce sufficient conditions that can be expressed structurally on game forms. Complement are given in Appendix~\ref{appen:correct_gf}.
%some example of simple sufficient conditions for game forms to be correct. 

Consider a game form $\formNF% = \langle \St_\A,\St_\B,\outComeNF,\outCNF \rangle
$, a partial valuation $\alpha: \outComeNF \setminus E \rightarrow [0,1]$ of the outcomes and assume that $v_\alpha > 0$. Consider some $v < v_\alpha$ and any optimal strategy $\sigma_\A \in \Opt_\A(\gameNF{\formNF}{\alpha[v]})$% in the game form $\formNF$ w.r.t. $\alpha[v]$
. We have $\va_{\gameNF{\formNF}{\alpha[v]}}(\sigma_\A) = f^\formNF_\alpha(v) > v$ (as $v_\alpha$ is the least fixed point of the function $f^\formNF_\alpha$). Hence, for all $b \in \St_\B$, we have $\delta(\Supp(\sigma_\A),b) \not \subseteq E$ (otherwise we would have $\outM_{\gameNF{\formNF}{\alpha[v]}}(\sigma_\A,b) = v$ since $\alpha[v][E] = \{ v \}$). Therefore, if an optimal strategy in $\formNF$ w.r.t. the valuation $\limval{\alpha} = \alpha[v_\alpha]$ can be found among the optimal strategies in $\formNF$ w.r.t. a valuation $\alpha[v]$ for some $v < v_\alpha$, then the game form $\formNF$ is correct w.r.t. $\alpha$. In particular, this is ensured for all partial valuations $\alpha$ as soon as there exists a finite set of strategies for Player $\A$ among which optimal strategies can be found w.r.t. any valuation.
%such that, for any valuation of the variables, an optimal strategy w.r.t. that valuation can be found in that set of strategies. 
This is stated in the proposition below.
%For the game form $\formNF$ not to be correct w.r.t. the partial valuation $\alpha$, there need to be a discontinuity of the maximal support of Player $\A$. 
%The least fixed point $v_\alpha$ of the function $f_\alpha^\formNF: [0,1] \rightarrow [0,1]$ (defined in Definition~\ref{def:partial_assignment}) is such that, for all $v < v_\alpha$, we have $v < f_\alpha(v)$. Interestingly, any optimal strategy $\sigma \in \Opt_\A(\langle \formNF,\limval{\alpha} \rangle)$ is such that $v \leq \va_{\langle \formNF,\alpha[v] \rangle}(\sigma)$ for all $v < v_\alpha$. However, only progressive strategy $\sigma$ in $\langle \formNF,\alpha[v] \rangle$ (that is, ensuring $\outCNF(\Supp(\sigma_\A),b) \not \subseteq E$ for all $b \in B$) is such that $v < \va_{\langle \formNF,\alpha[v] \rangle}(\sigma)$ for all $v < v_\alpha$ (since $\alpha[v][E] = \{ v \}$). This gives another characterization of correct strategy w.r.t. a partial valuation in the proposition below. 
%\begin{proposition}[Correct game forms w.r.t. a partial valuation]
%	\label{def:correct_gf_partial_valuation_other}
%	Consider a game form $\formNF = \langle \St_\A,\St_\B,\outComeNF,\outCNF \rangle$ and a partial valuation of the variable $\alpha: \outComeNF \setminus E \rightarrow [0,1]$ for some subset of outcomes $E \subseteq O$. 
%	The game form $\formNF$ is \emph{correct} w.r.t. the partial valuation $\alpha$ if and only if there exists a strategy $\sigma \in \Dist(A)$ such that, for all $v < v_\alpha$, $v < \va_{\langle \formNF,\alpha[v] \rangle}(\sigma)$.
%\end{proposition}

%It follows that if a finite number of strategies if sufficient to increase the value of the game, then the game form is correct.
\begin{proposition}
	\label{prop:finite_number_strat_sufficient}
	For a game form $\formNF% = \langle \St_\A,\St_\B,\outComeNF,\outCNF \rangle
	$, assume that there exists a finite set $S \subseteq \Dist(A)$ of strategies for Player $\A$ such that, for all %(total) 
	valuations $v \in [0,1]^\outComeNF$, there exists an optimal strategy for Player $\A$ in $S$: $\Opt_\A(\gameNF{\formNF}{v}) \cap S \neq \emptyset$. Such a game form is called a \emph{finite-set} game form. 
	In that case, the game form $\formNF$ is correct.%for all partial valuation $\alpha$ and $v < v_\alpha$, then there exists $\sigma_\A \in S$ such that $v < v_\alpha$, $v < \va_{\langle \formNF,\alpha[v] \rangle}(\sigma)$. Then, the game form $\formNF$ is correct. Note that it holds in particular in the case where, for all valuations $v \in \outComeNF^{[0,1]}$, there exists an optimal strategy for Player $\A$ in $S$: $\Opt_\A(\langle \formNF,v \rangle) \cap S \neq \emptyset$.
\end{proposition}

\begin{figure}
	\begin{minipage}[b]{0.32\linewidth}
		\centering
		\includegraphics[scale=0.8]{Tex/Figure/FormNF/formNFCircular1.pdf}
		\caption{A circular game form.}
		\label{fig:circular_gf}
	\end{minipage}
	\begin{minipage}[b]{0.32\linewidth}
		\centering
		\includegraphics[scale=0.9]{Tex/Figure/FormNF/formNFDet1.pdf}
		\caption{A determined game form $\formNF$.}
		\label{fig:det_gf}
	\end{minipage}
	\begin{minipage}[b]{0.32\linewidth}
		\centering
		\includegraphics[scale=0.9]{Tex/Figure/FormNF/formNFDet2.pdf}
		\caption{The game in normal form $\gameNF{\formNF}{v}$ with $v(x) = 0,v(y) = 1, v(z) = 0$.%There is a column of $0$s.
		}
		\label{fig:valued_det_gf}
	\end{minipage}
\end{figure}

Let us now exhibit some finite-set game forms. Consider a game form $\formNF$ with only two outcomes $x$ and $y$. Then, an optimal strategy in $\formNF$ w.r.t. to a valuation $v$ of $x$ and $y$ can be chosen by only knowing whether $v(x) < v(y)$ or not. %An example is given in Figure~\ref{fig:}. 
Hence, such game forms are finite-set. %Hence, two-variable game forms satisfy the premise of Proposition~\ref{prop:finite_number_strat_sufficient}. 
Furthermore, there are game forms such that a strategy (playing uniformly over all actions) is optimal regardless of the valuation considered: this is the case of \emph{circular} game forms where the columns correspond to all the permutations of the first column, an example is given in Figure~\ref{fig:circular_gf}. Such game forms are also finite-set. %Such game forms are correct, by Proposition~\ref{prop:finite_number_strat_sufficient}. 
Finally, some game forms only require deterministic strategies to play optimally. This, in fact, characterize the \emph{determined} game forms which are the game form $\formNF$ ensuring that, for all $0-1$ valuations $v: \outComeNF \rightarrow \{ 0,1 \}$ of the variables, there is either a line of 1 or a column of 0 in the resulting game in normal form $\gameNF{\formNF}{v}$. An example of determined game form is given in Figure~\ref{fig:det_gf} with an example of valuation in Figure~\ref{fig:valued_det_gf}. Determined game forms are also finite-set.
These results are stated in the proposition below.
\begin{proposition}
	\label{prop:some_correct_game_forms}
	Consider a game form $\formNF$. The game form $\formNF$ is correct as soon as either $|\outComeNF| \leq 2$ or $\formNF$ is a circular game form or $\formNF$ is a determined game form.
\end{proposition}

\smallskip \noindent \textbf{Determined game forms and correct game forms.}
Determined game forms have been studied in (ref). The authors have shown, via an equivalence with turn-based game, that these game forms exactly correspond to the ones ensuring that, when used as local interactions of concurrent deterministic games (for arbitrary Borel winning set), both players have deterministic winning strategies. In fact, when the game is stochastic, this equivalence still holds. It follows that, as reachability turn-based games are positionally determined (ref), so are reachability games with determined local interactions. This result, combined with Theorem~\ref{thm:main} gives immediately that determined game forms are correct. Interestingly, determined game forms are also characterized with the least fixed point operator as in the proposition below.%: they correspond to game forms where the valuation of a partial valuation given by the functiononly one iteration of the function is necessary to reach the limit valuation. This is stated in the proposition below.
\begin{proposition}
	A game form $\formNF% = \langle \St_\A,\St_\B,\outComeNF,\outCNF \rangle
	$ is \emph{determined} if and only if, for all partial valuations $\alpha: \outComeNF \setminus E$ of the variables, we have $v_\alpha = f^\formNF_\alpha(0)$.
\end{proposition}

%Finally, finite-set game forms can be combined to obtain new finite-set game forms.
%\begin{proposition}
%	Consider a finite-set game form $\formNF$. If all its outcomes in $\outComeNF$ are replaced by other finite-set game forms (the same outcomes being replaced by the same game forms), the resulting game forms is also finite-set.
%\end{proposition}

%\textbf{Two-variables game forms} Consider the game forms in Figure~\ref{fig:two_var_gf}. The one on the left corresponds to the classic matching pennies game: regardless of the valuation, playing both lines with probability $1/2$ induces an optimal strategy for Player $\A$. An optimal strategy in the game form in the middle consists in playing the right or bottom line with probability $1$ depending on whether or not $x < y$. Finally, the outcome of a game in normal form obtained from the game form on the right for any valuation in independent of the strategy chosen by Player $\A$. In fact, any game form with at most two variables is a finite-set game form, as stated in the proposition below.
%\begin{figure}
%	\begin{minipage}[b]{0.32\linewidth}
%		\centering
%		\includegraphics[scale=0.9]{Tex/Figure/FormNF/formNF2var1.pdf}
		%\caption{}
		%\label{fig:one_state}           
%	\end{minipage}
%	\begin{minipage}[b]{0.32\linewidth}
%		\centering
%		\includegraphics[scale=0.9]{Tex/Figure/FormNF/formNF2var2.pdf}
		%\caption{}
		%\label{fig:one_state}           
%	\end{minipage}
%	\begin{minipage}[b]{0.32\linewidth}
%		\centering
%		\includegraphics[scale=0.9]{Tex/Figure/FormNF/formNF2var3.pdf}
		%\caption{}
		%\label{fig:one_state}           
%	\end{minipage}
%	\caption{Three examples of two-variables game forms.}
%	\label{fig:two_var_gf}
%\end{figure}

%\begin{proposition}
%	\label{prop:two_var_gf}
%	Any game form $\formNF = \langle \St_\A,\St_\B,\outComeNF,\outCNF \rangle$ such that $|\outComeNF| \leq 2$ is correct. 
%\end{proposition}

%\textbf{Determined game forms.} The finite set of strategies among which optimal strategies can be found regardless of the valuation considered can be the set of deterministic strategies. In fact, this characterizes exactly the \emph{determined} game forms, defined below.
%\begin{figure}
%	\begin{minipage}[b]{0.49\linewidth}
%		\centering
%		\begin{minipage}[b]{0.22\linewidth}
%			\centering
%			\includegraphics[scale=0.9]{Tex/Figure/FormNF/formNFDet1.pdf}      
%		\end{minipage}
%		\hspace*{0.5cm}
%		\begin{minipage}[b]{0.22\linewidth}
%			\centering
%			\includegraphics[scale=0.8]{Tex/Figure/FormNF/formNFDet2.pdf}      
%		\end{minipage}
%		\caption{Two determined game forms.}
%		\label{fig:det_gf}
%	\end{minipage}
%	\begin{minipage}[b]{0.49\linewidth}
%		\centering
%		\begin{minipage}[b]{0.22\linewidth}
%			\centering
%			\includegraphics[scale=0.8]{Tex/Figure/FormNF/formNFCircular1.pdf}
%		\end{minipage}
%		\hspace*{0.5cm}
%		\begin{minipage}[b]{0.25\linewidth}
%			\centering
%			\includegraphics[scale=0.8]{Tex/Figure/FormNF/formNFCircular2.pdf} 
%		\end{minipage}
%		\caption{Two circular game forms.}
%		\label{fig:circular_gf}
%	\end{minipage}
%\end{figure}

%\begin{definition}
%	A game form $\formNF = \langle \St_\A,\St_\B,\outComeNF,\outCNF \rangle$ is \emph{determined} if, for any $0-1$-valuation $v: \outComeNF \rightarrow \{ 0,1 \}$ of the variables, there is either a row of 1s or a column of 0s in $\langle \formNF,v \rangle$.
%\end{definition}
%Examples of determined game forms can be found in Figure~\ref{fig:det_gf}. Such game forms have been studied in \ref{}: the authors have proved that they exactly correctly correspond to the game forms that ensure that all concurrent stochastic game with a Borel objective using them as local interactions is determined. Interestingly, such game forms can also be characterized with the least fixed point operator: they correspond to game forms where only one iteration of the function is necessary to reach the limit valuation. This is stated in the proposition below.
%\begin{proposition}
%	A game form $\formNF% = \langle \St_\A,\St_\B,\outComeNF,\outCNF \rangle	$ is \emph{determined} if and only if, for all partial valuation $\alpha: \outComeNF \setminus E$ of the variables, we have $\limval{\alpha} = f^\formNF_\alpha(0)$.
%\end{proposition}

%By definitions, such game forms are correct.
%\begin{proposition}
%	Any determined game form is correct.
%\end{proposition}

%\textbf{Circular game forms.} Finally, in the case the finite set of strategies sufficient to find optimal strategies can be a singleton, the corresponding strategy should be a uniform strategy: all actions are assigned the same probability. For such a strategy to always be optimal, the columns of that game forms should be a circular permutation of one another. Examples of such game forms are given in Figure~\ref{fig:circular_gf}. 
%all lines in the game form should have the same variables, counted with multiplicity. This induces the definition of \emph{circular} game form below.

%\begin{definition}
%	A game form $\formNF = \langle \St_\A,\St_\B,\outComeNF,\outCNF \rangle$ is said to be \emph{circular} if, for all $b,b' \in \St_\B$, there exists a bijection $\sigma: \St_\A \rightarrow \St_\A$ such that, %there exists $n \in \N$ and a bijection $f: \St_\A \rightarrow \llbracket 1,n \rrbracket$ such that:
	%\begin{itemize}
	%	\item $n = |\St_\A| = |\St_\B|$;
	%	\item for all $b,b' \in \St_\B$, there exists a permutation $\sigma: \llbracket 1,n \rrbracket \rightarrow \llbracket 1,n \rrbracket$ such that, 
%	for all $a \in \St_\A$, we have $\outCNF(a,b) = \outCNF(\sigma(a),b')$.
	%\end{itemize}
%\end{definition}

%\begin{proposition}
%	Any circular game form is correct.
%\end{proposition}

\smallskip \noindent \textbf{Decision problem.} Finally, consider the problem of deciding whether a given game form is correct. Deciding this problem with a standard algorithm is not direct as the definition of correct game forms involves a universal quantification and a least fixed point operator. However, this can done straightforwardly by using the theory of the reals: the correctness of game forms can be expressed with universal and existential quantifiers over the valuations, support, and strategies considered. This induces the proposition below.
\begin{proposition}[Proof~\ref{proof:decidability}]
	\label{prop:decidability}
	The correctness of game forms is decidable.
\end{proposition}



==> Tex/ValueLFP.tex <==
%!TEX root = ../lipics-v2021-sample-article

Let $\langle \Aconc,T \rangle$ be concurrent stochastic reachability game% that we will consider throughout this section with $\Aconc = \AConc$
. W.l.o.g. we assume that all states $q \in T$ are self-looping sinks. The distance $\dNorm_{|Q|}$ is denoted $\dNorm$. By Martin's theorem (ref?), we know that this game has a value from each state. However, in the particular case of a reachability game, this value is given by the least fixed point of an operator on states (ref?). In this section, we recall the definition of this operator and give proof sketches that the value of the game is indeed given by its least fixed point.
%This section is devoted to the proof of the following existing result: in any finite concurrent stochastic reachability game, optimal strategies exist among positional strategies for Player $\B$ (Player {\sf Min} in the literature). 
%The proof is mainly based on an operator on value that will be iterated whose limit will be the value of the game. We consider the following definitions.

Let us first introduce a notation to lift a valuation of the states to a valuetion of the Nature states via a convex combination.
\begin{definition}[Valuation of the Nature states]
	For a valuation $v \in [0,1]^Q$ of the states, we define the valuation $\mu_v \in [0,1]^\distribSet$ of the Nature states by $\mu_v(d) := \sum_{q \in Q} \distribFunc(d)(q) \cdot v(q)$ for all $d \in \distribSet$.
\end{definition}

We can now define the operator on vectors of values on the states whose least fixed point gives the value of the game.
\begin{definition}[Operator on values and latiice]
	\label{def:operator}
	Let $\Delta: [0,1]^Q \rightarrow [0,1]^Q$ be such that, for all valuations $v \in [0,1]^Q$ and $q \in Q$, we have $\Delta(v)(q) := \va_{\langle \formNF_q,\mu_v \rangle}$ if $q \notin T$ and $\Delta(v)(q) := 1$ otherwise. Let also $V = \{ v \in [0,1]^Q \mid \forall q \in T,\; v(q) = 1 \} \subseteq [0,1]^Q$ be a set of valuations..
\end{definition}

%Finally, we define a set of valuations %and a binary relation on this set that will, in turn, induce a complete lattice with the binary relation $\preceq$ defined in the preliminaries.
%\begin{definition}
%	We consider the set of valuations $V = \{ v \in [0,1]^Q \mid \forall q \in T,\; v(q) = 1 \} \subseteq [0,1]^Q$.
%\end{definition}

These definitions ensure the proposition below.
\begin{proposition}[Proof~\ref{proof:proposition_property_Delta}]
	\label{prop:property_Delta}
	The operator $\Delta$ and the set $V$ ensure the following properties:
	\begin{enumerate}
		\item $(V,\preceq)$ is a complete lattice with minimal element denoted $v_0$;
		\item $\Delta[V] \subseteq V$ and $\Delta$ is non-decreasing%: if $v \preceq v'$, then $\Delta(v) \preceq \Delta(v')$
		;
		\item $\Delta$ is 1-Lipschitz w.r.t. the distance $\dNorm$%_{|Q|}
		(only continuity is necessary for what follows).
	\end{enumerate}
\end{proposition}

The value of the game is now given by least fixed point of the function $\Delta$ on $V$. 

\begin{definition}
	Let $\textsf{m}_{\Delta}$ be the least fixed point of the function $\Delta$ on $V$. Note that its existence is ensured by Knaster-Tarski (ref?) theorem with points $1$ and $2$.
\end{definition}

Before proving that, for all $q \in Q$, we have $\textsf{m}_{\Delta}(q) = \val{\Aconc}{}(q)$ ,we state a useful proposition below stating that the probability to reach the target set of states $T$ in at most $n$ steps can be expressed inductively.
\begin{proposition}[Proof~\ref{proof:rmq_relation_proba}]
	\label{rmq:relation_proba}
	Consider two strategies $\s_\A,\s_\B \in \SetStrat{\Aconc}{\A} \times \SetStrat{\Aconc}{\B}$ for Player $\A$ and $\B$ and  a state $q \in Q \setminus T$. Then, we have the following relation% (recall that residual strategies $\s_\A^q$ and $\s_\B^q$ are defined in Definition~\ref{def:value_graph_game})
	:
	\begin{displaymath}
	\prob{n+1}{\s_\A}{\s_\B}(q,T) = \sum_{q' \in Q}
	\prob{q,q'}{}{}(\s_\A(q),\s_\B(q)) \cdot \prob{n}{\s_\A^q}{\s_\B^q}(q,T)
	\end{displaymath}
\end{proposition}

Now, we state in the lemma below that Player $\B$ has a positional strategy $\s_\B$ whose value is less than or equal to $\mathsf{m}_\Delta(q)$ from all state $q \in Q$.
\begin{lemma}
	\label{lem:leq_m_delta}
	Consider a concurrent stochastic game $\langle \Aconc,T \rangle$ with $\Aconc = \AConc$ and $\Delta: [0,1]^Q \rightarrow [0,1]^Q$ the operator on values defined in Definition~\ref{def:operator}. There exists a positional strategy $\s_\B \in \SetPosStrat{\B}{\Aconc}$ for Player $\B$ such that, for all $q \in Q$: $\val{\Aconc}{\s_\B}(q) \leq \mathsf{m}_\Delta(q)$.
\end{lemma}
\begin{proofs}[Complete Proof~\ref{proof:leq_m_delta}]
	
\end{proofs}

The case of Player $\A$ is not symmetric as she does not have an optimal strategy in th general case (cf boule de neige), however, for all $\varepsilon > 0$, she has strategies realizing the value $\mathsf{m}_\Delta(q) - \varepsilon$ from all state $q \in Q$. This is stated in the lemma below. 

\begin{lemma}
	\label{lem:geq_m_delta}
	Consider a concurrent stochastic game $\langle \Aconc,T \rangle$ with $\Aconc = \AConc$ and $\Delta: [0,1]^Q \rightarrow [0,1]^Q$ the operator on values defined in Definition~\ref{def:operator}. For all $\varepsilon > 0$, there exists a strategy $\s_\A \in \SetPosStrat{\A}{\Aconc}$ for Player $\A$ such that, for all $q \in Q$: $\val{\Aconc}{\s_\A}(q) \geq \mathsf{m}_\Delta(q) - \varepsilon$. It follows that, for all $q \in Q$: $\val{\Aconc}{\A}(k) \geq \mathsf{m}_\Delta(q)$.
\end{lemma}
\begin{proofs}[Complete Proof~\ref{proof:geq_m_delta}]
	
\end{proofs}

Overall, the value of the game is given by $\mathsf{m}_\Delta$, as stated in the theorem below.
\begin{theorem}
	\label{thm:m_delta}
	Consider a concurrent stochastic game $\langle \Aconc,T \rangle$ with $\Aconc = \AConc$ and $\Delta: [0,1]^Q \rightarrow [0,1]^Q$ the operator on values defined in Definition~\ref{def:operator}. For all $q \in Q$, we have: $\mathsf{m}_\Delta$ of $\Delta$: $\val{\Aconc}{}(q) = \mathsf{m}_\Delta(q)$. Furthermore, there exists a positional strategy $\s_\B \in \SetPosStrat{\B}{\Aconc}$ for Player $\B$ ensuring, for all $q \in Q$, $\val{\Aconc}{\s_\B}(q) = \val{\Aconc}{}(q)$.
\end{theorem}
\begin{proof}
	This is a direct consequence of Lemmas~\ref{lem:leq_m_delta} and~\ref{lem:geq_m_delta}.
\end{proof}
